Geodesic-HOF: 3D Reconstruction Without Cutting Corners

Single-view 3D object reconstruction is a challenging fundamental problem in computer vision, largely due to the morphological diversity of objects in the natural world. In particular, high curvature regions are not always captured effectively by methods trained using only set-based loss functions, resulting in reconstructions short-circuiting the surface or cutting corners. In particular, high curvature regions are not always captured effectively by methods trained using only set-based loss functions, resulting in reconstructions short-circuiting the surface or cutting corners. To address this issue, we propose learning an image-conditioned mapping function from a canonical sampling domain to a high dimensional space where the Euclidean distance is equal to the geodesic distance on the object. The first three dimensions of a mapped sample correspond to its 3D coordinates. The additional lifted components contain information about the underlying geodesic structure. Our results show that taking advantage of these learned lifted coordinates yields better performance for estimating surface normals and generating surfaces than using point cloud reconstructions alone. Further, we find that this learned geodesic embedding space provides useful information for applications such as unsupervised object decomposition.

==> introduction_old.tex <==
\section{Introduction \volkan{[]}}
\eric{General comment: I think this intro does great exposition, but could have a stronger narrative. We could establish more strongly specific shortcomings in existing methods and why our method is a logical way of addressing them. The key question that I don't think is currently answered is: \textit{Why learn geodesics?}}

Reconstructing the 3D model of an object from a single image is a central problem in computer vision. It is challenging because building a complete 3D model requires reasoning about the occluded parts of the object as well as the depth of the pixels which correspond to the visible part. \eric{These things are challenging, but they aren't challenges that we are specifically address here. I think we should emphasize the challenges that we're taking on}

Recent deep learning based approaches have shown  promise in addressing these challenges.
A key decision in designing a network for 3D shape representation is the object representation. It has been shown that deep learning architectures, once trained on large datasets such as ShapeNet~\cite{}, are capable of outputting accurate object models represented as voxels~\cite{} or point clouds~\cite{}.

\eric{I think we can boil this down to one sentence, and include it as motivation in the first paragraph}
There are many applications which require continuous surface representations. For example, in computer graphics, surface models such as triangle meshes are used for computing object appearance. In robotics, surface normals are used for grasp planning. In computer aided design and manufacturing, complete object models are needed for production e.g., for 3D printing. Therefore significant recent research effort in 3D object reconstruction has been dedicated to approaches which can generate continuous surface models. 

\eric{I think this is a better fit for related work}
% In principle, surface normals can be estimated from local Euclidean neighborhoods. Therefore, surfaces can be generated by coupling methods capable of generating dense point-clouds such as~\cite{mitchell2019higher} with surface reconstruction algorithms such as Poisson Surface Reconstruction~\cite{kazhdan2006poisson}. However, these methods do not yield accurate results in high curvature areas even for simple objects.  As an alternative, methods such as Atlas-Net~\cite{atlasnet} and Pixel2Mesh~\cite{wang2018pixel2mesh} which are capable of directly outputting surface representations have been developed. The main idea in Atlas-Net is to deform a sheet (i.e., a 2D manifold) onto the surface of the object by minimizing Chamfer distance. However, a single sheet may not be sufficient to cover a complex shape. Therefore, a large number of sheets are sometimes needed to obtain accurate results. The number and initialization of these sheets is somewhat arbitrary. Overlaps across the sheets after warping  need to be handled separately. Pixel2Mesh overcomes this issue by warping a triangulation of the sphere surface using graph convolutions. These methods have been recently extended \volkan{maybe a sentence about atlasnet2, pixel2mesh++, mesh-rcnn} Such methods can produce objects with a fixed, typically genus zero, topology.

% \eric{Also better for related work?}
% Alternatively, implicit functions such as occupancy~\cite{mescheder2019occupancy} or signed distance~\cite{park2019deepsdf} which are continuous by definition have been explored as object representations. One of the main drawbacks of such methods is the need for a post-processing step such as running marching cubes to generate the object. Furthermore, generating training data for these methods is non-trivial since they require dense samples near the surface of the object. Finally, \volkan{as noted in~\cite{mescheder2019occupancy}?}, in terms of Chamfer score, implicit function methods are not as accurate as \emph{direct methods} such as AtlasNet and Pixel2Mesh which are trained directly using  Chamfer-based loss functions. 

\volkan{let's revisit the notation and labels below ($f$ vs. $g$ etc) once we finalize the figures and sections.}

In this paper, we present a new direct method for reconstructing a continuous surface representation of an object from a single image. Our method is based on two key ideas. First, rather than relying on a fixed resolution output, we represent the object as a mapping function $f: S \rightarrow \R^d$ where $S$ is the unit sphere.  The mapping function $f$ is represented as a neural network whose weights are computed from an input RGB image by a second, ``higher order" function (HOF). Second, rather than mapping points to $\R^3$ where the object surface lies, $f$ maps points in $S$ to $\R^d$, $d > 3$  in such a way that the \emph{Euclidean} distance between two points after the mapping corresponds to their geodesic distance on the object surface. We call this architecture \ours and 
 show that by learning geodesic distances, \ours learns surface features such as curvature which are not easily captured by point-set distance functions such as Chamfer. 



We showcase the performance of \ours in three settings. In Section~\ref{sec:x1}, we compare \ours with state of the art direct mapping methods such as Atlas-Net and Pixel2Mesh and show that \ours outperforms them both in terms of Chamfer distance and accuracy of surface normals. Next, we compare \ours with implicit function methods such as Occupancy Net, and \ours achieves lower Chamfer distance. This experiment highlights the tradeoff made in baseline methods that use Marching Cubes in post-processing, which enhances surface normal accuracy at the expense of loss of surface detail.
% Despite Chamfer accuracy, the smoothing which comes from the marching-cubes post-processing gives impicit function methods an edge in terms of normal accuracy. 
% Yet, \ours is only slightly worse and has the advantage of producing a direct mapping  onto the object surface. 
Finally, in Section~\ref{sec:x3}, we show how the learned representation can be used for meaningful object decompositions into non-overlapping 2d-manifolds which can be used for generating triangulations or explicit function representations of surfaces. 

\volkan{maybe we should show the cube, the table and the swiss roll here and explicity mention them.}

\volkan{we may want to change the tone of this last paragraph and only mention the experiments; and present the conclusions after the experiments. }
\eric{I made some tone changes}


